Chasing Random: Instruction Selection Strategies Fail to Generalize

Prior work has shown that language models can be tuned to follow user instructions using only a small set of high-quality instructions. This has accelerated the development of methods that filter a large, noisy instruction-tuning datasets down to high-quality subset which works just as well. However, typically, the performance of these methods is not demonstrated across a uniform experimental setup and thus their generalization capabilities are not well established. In this work, we analyze popular selection strategies across different source datasets, selection budgets and evaluation benchmarks: Our results indicate that selection strategies generalize poorly, often failing to consistently outperform even random baselines. We also analyze the cost-performance trade-offs of using data selection. Our findings reveal that data selection can often exceed the cost of fine-tuning on the full dataset, yielding only marginal and sometimes no gains compared to tuning on the full dataset or a random subset.

==> cost-estimation.tex <==
\setlength{\tabcolsep}{4pt} 
\begin{table*}[]
\small 
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{cccclcccll}
\toprule
\rowcolor[HTML]{CBCEFB} 
\textbf{Dataset} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Samples \\ (as multiples \\ of 1k)\end{tabular}} &
  \textbf{Alpacasus} &
  \multicolumn{3}{c}{\cellcolor[HTML]{CBCEFB}\textbf{Cherry}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{CBCEFB}\textbf{DEITA}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{CBCEFB}\textbf{\begin{tabular}[c]{@{}c@{}}Entire\\ Dataset\end{tabular}}} \\ 
  \midrule
\textbf{\begin{tabular}[c]{@{}c@{}}Costing \\ Categories\end{tabular}} &
   &
  {\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}API Inference \\ Cost (USD)\end{tabular}} &
  \multicolumn{2}{c}{{\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}Rent Time\\ (min)\end{tabular}}} &
  {\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}Rent Cost \\ (USD)\end{tabular}} &
  {\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}Rent Time \\ (min)\end{tabular}} &
  {\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}Rent Cost\\ (USD)\end{tabular}} &
  \multicolumn{1}{c}{{\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}Rent Time\\ (min)\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{343434} \begin{tabular}[c]{@{}c@{}}Rent Cost\\ (USD)\end{tabular}}} \\ 
EVOL &
  200 &
  \cellcolor[HTML]{CBCEFB}50 &
  \multicolumn{2}{c}{3290} &
  \cellcolor[HTML]{CBCEFB}427 &
  1000 &
  \cellcolor[HTML]{CBCEFB}130 &
  1620 &
  \cellcolor[HTML]{CBCEFB}216 \\
ALPACA &
  52 &
  \cellcolor[HTML]{CBCEFB}12.66 &
  \multicolumn{2}{c}{855} &
  \cellcolor[HTML]{CBCEFB}{\color[HTML]{000000} 111.15} &
  260 &
  \cellcolor[HTML]{CBCEFB}33.8 &
  120 &
  \cellcolor[HTML]{CBCEFB}15.6 \\
DOLLY &
  15 &
  \cellcolor[HTML]{CBCEFB}3.7 &
  \multicolumn{2}{c}{246.75} &
  \cellcolor[HTML]{CBCEFB}32.07 &
  75 &
  \cellcolor[HTML]{CBCEFB}9.975 &
  40 &
  \cellcolor[HTML]{CBCEFB}5.2 \\
FLAN &
  88 &
  \cellcolor[HTML]{CBCEFB}21.46 &
  \multicolumn{2}{c}{1447.6} &
  \cellcolor[HTML]{CBCEFB}188.2 &
  440 &
  \cellcolor[HTML]{CBCEFB}57.2 &
  220 &
  \cellcolor[HTML]{CBCEFB}28.6 \\\hline
\end{tabular}
\label{tab:cost-estimates}
\end{adjustbox}
\caption{The effective cost of data selection is non-trivial in comparison to training on the full-dataset. In three out of four strategies, it is possible to overshoot the cost of finetuning on the full dataset and this does not even include the cost of hyperparameter tuning for optimizing on the performance of the selection strategy.  
\textcolor{purple}{Check the cost of Alpacasus - Was this on the whole dataset ?}}
\end{table*}
\section{Documenting the Cost of Selection}

A strong motivation for designing instruction selection strategies, and more broadly, data selection strategies draws from the need to train competitive models efficiently, both in terms of cost and resource consumption. While the reduction in training on subsampled data is more explicitly observeable at larger scales of data selection (in pretraining data selection, for example), instruction tuning datasets are typically signficantly smaller in order of magnitude and thus the cost effectiveness of subsampling can be less obvious to gauge. Accordingly, we evaluate if the proposed selection strategies consistently provide that intended benefit by observing the effective cost of selection against the performance gained through selection. 

\paragraph{Infrastructure:} All our estimates are provided assuming the following infrastructure: 8 A6000s, 128 CPUs provided by \href{https://cloud.google.com/compute/all-pricing}{Google Cloud Estimator}. The Dollar Cost of renting our infrastructure per hour is about 8 USD.


\begin{figure*}[h]
    \centering
    \small
    \includegraphics[width=0.9\linewidth]{assets/cost_versus_performance_correlation@1k.pdf}
    \caption{Cost Versus Performance Trade-Off at Selection Budget of 1000: (These are the costs of selecting a 1000 datapoints using the said selection strategy and only the \textbf{lowest} performance amongst all our random trials is chosen to give the most pessimistic estimate of the performance of our random baseline as well as a lower-bound on the cost of the selection strategy. Note that since the entire dataset needs to be scored in accordance with a selection strategy's heuristic irrespective of the final sampling budget - the total cost of selection does not vary signficantly with the change in the sampling budgets that we consider)  }
    \label{fig:cost-performance-correlation}
\end{figure*}

\paragraph{Cost Calculation:} We define the Effective Cost of Selection as the combined cost of applying the selection strategy on a given dataset. To do this, we take a product of the per-hour cost to user for renting our stated compute infrastructure and our wall clock run time for running the selection for a strategy end-end.  The wall clock of running each selection is described in \ref{wall-clock-time}, while the total cost to user in summarized in \ref{tab:cost-estimates}.

% and (b) the cost of finetuning on the selected dataset of a fixed budget. While the latter might seem degenerate to account for as the cost of finetuning on a dataset for a fixed budget doesn't vary per strategy - we argue that it is important to consider this cost as a part of the selection cost as we cannot conclude the efficacy of a selection strategy without incurring this finetuning cost.


% For comparison with effective cost of finetuning (including read/write operations for saving model checkpoints and tokenization and training run) is constant for a fixed budget for the selected data runs (10000 samples) and comes to 1hr 13 mins on our setup. For comparison with the effective cost of finetuning on the entire dataset, we similarily compute the full finetuning costs 



\hdtodo{In the cost that is being expended to do the data selection, we can train x number of random baselines or y number of full finetuned models on different hyperparameter configurations (negating the need to tune for strategy specific parameters).}

\paragraph{Findings} The effective cost of tuning a model on selected data (cost of selection and finetuning on that subset) for most of the studied strategies is not trivial in relative comparison to the full-finetuning cost for some strategies. Since these are only single runs, these costs also don't account for any hyperparameter tuning that might have been applied by the designers of the strategy for best performance at a given combination of budget and dataset. This is especially problematic for 2 reasons: Firstly, in instruction data selection, we can optimize 2 kind of hyperparameters: (a) traditional model training parameters like learning rate, scheduler and batch size and (b) instruction-selection strategy dependent parameters such as the similarity threshold, $\lambda$ in DEITA, the number of pre-experienced samples in Cherry, etc. Jointly optimizing for both these class of hyperparameters can significantly bloat the set of combinations to explore for hyperparameter optimization. Secondly, under a practical setup where an NLP pracitioner expects to choose the best selection strategy \textit{amongst} several candidate strategies, a hyperparameter sweep for each candidate strategy would mandate tuning \textbf{all the strategies being examined}. From \ref{tab:cost-estimates}, this would imply summing the cost estimates across any row. We can clearly see that such an estimate would quickly overshoot the cost of full finetuning for any strategy. 


% Overall, the variation in the performance of all selection strategies observed through evaluations on OpenLLM, IFFEval and AlpacaEval2.0 indicate that strategies would have such a strong dependence on hyperparameters to give significant and consistent gains over random sampling, and the cost of selection itself may make this relatively hard to afford. 

 % For example - \textcolor{purple}{add the plot comparing FLAN on h3 and h2: Both hyperparameters are adopted in the literature but in h3: all strategies significantly outperform bad-random (i.e., complement selection is also useful there) while on H2 }

\paragraph{Estimating Performance Using Cost-Effective Proxies} 

While it is not possible to largely modify the cost of a selection strategy, it might be possible to offset the cost of finetuning the models on subsets generated via different selection strategies through parameter efficient techniques. If such trends are correlated with the performance of the selected data on the full variant of the model, NLP practioners can potentially design a set of relatively low-cost experiments to rapidly identify the optimal selection strategy to further carry out their selection. Recent work like \cite{Xia2024LESSSI}, even leverage such correlation to achieve great efficiency in task-specific instruction selection. For preliminary experimentation, we rerun all our experiments with the modification of including LORA modules in our finetuning. This reduces the memory footprint of training by to only 0.0038 times of the memory footprint of full finetuning along with faster training by half of its full-finetuning counterpart. In \ref{fig:lora-fft-correlation} we plot the correlation between the instruct-level-accuracy on IFFEVAL for models trained with and without LORA. However, we don't find any reasonable correlation between these performances highlighlting a need to identify cost-effective methods of predicting the suitability of a custom budget and source distribution to a given selection strategy. 


\begin{figure}[h]
    \small
    \centering \includegraphics[width=0.5\linewidth]{assets/correlation_btw_lora_fft.pdf}
    \caption{There isn't any observable correlation between the performance of models finetuned with and without LORA across our setups indicating that we cannot reliably predict the optimal selection strategy on a faster, cost-effective parameter efficient setup.}
    \label{fig:lora-fft-correlation}
\end{figure}



